Exploration of Nuclear Matter Properties and Related Thermodynamical Aspects

In this study, my main goal is to examine the nuclear matter properties across a wide range of conditions, such as temperature, density, asymmetry, pressure, and magnetic field. Understanding the effect of these factors on nuclear matter is essential, given their relevance in various phenomena such as heavy-ion collisions, neutron stars, and supernovae. However, due to the absence of a fundamental nuclear theory, we must rely on models to describe the nuclear matter. Predicted properties like neutron star mass-radius relationships, tidal deformability, structure, critical points in the nuclear matter phase diagram etc. depend on the chosen model. This dependence arises because key parameters characterizing any nuclear model or equation of state (EoS) are not precisely known. Therefore, it is crucial to investigate how nuclear matter properties behave under various conditions and in relation to different EoS parameters. To accomplish this, I have examined three distinct forms of nuclear matter: infinite nuclear matter, finite nuclei, and neutron stars, using the effective relativistic mean field model (E-RMF).

==> Chapter_7/table.tex <==
%%%%%%%%%%%%%%
\begin{comment}
\begin{table*}
\caption{The sequence of nuclei in the outer crust of neutron star from low to high density at various values of the magnetic field. The most recent experimental atomic mass evaluations AME2020 \cite{Huang_2021} are taken whenever available and microscopic calculations of HFB-24 and HFB-26 \cite{hfb2426} along with the FRDM(2012) mass table \cite{MOLLER20161} is used for the unknown mass. The nuclei marked with $^*$ and highlighted are the last nuclear species which are estimated from the experimental masses.}
\label{tab:nuc_seq}
\renewcommand{\arraystretch}{1.1}
\resizebox{\textwidth}{!}{%
\begin{tabular}{llllllllllllllll}
\hline
\hline
$B^*$ & \multicolumn{3}{c}{1000} & \multicolumn{3}{c}{2000} & \multicolumn{3}{c}{3000} & \multicolumn{3}{c}{4000} & \multicolumn{3}{c}{5000} \\
\hline
 S.N.  & HFB26   & HFB24  & FRDM       & HFB26    & HFB24     & FRDM      & HFB26      & HFB24     & FRDM      & HFB26     & HFB24    & FRDM     & HFB26      & HFB24      & FRDM  \\
   \hline
 1&$^{56}$Fe  &$^{56}$Fe  &$^{56}$Fe  &$^{56}$Fe  &$^{56}$Fe   &$^{56}$Fe  &$^{56}$Fe  &$^{56}$Fe  & $^{56}$Fe &$^{56}$Fe  &$^{56}$Fe &$^{56}$Fe  &$^{56}$Fe   & $^{56}$Fe  & $^{56}$Fe \\
 2&$^{62}$Ni  &$^{62}$Ni  &$^{62}$Ni  &$^{62}$Ni  & $^{62}$Ni  &$^{62}$Ni  &$^{62}$Ni  &$^{62}$Ni  & $^{62}$Ni &$^{62}$Ni  &$^{62}$Ni  &$^{62}$Ni  &$^{60}$Ni   & $^{60}$Ni  &$^{60}$Ni  \\
 3&$^{64}$Ni  &$^{64}$Ni  &$^{64}$Ni  &$^{88}$Sr  &$^{88}$Sr   &$^{88}$Sr  &$^{88}$Sr  &$^{88}$Sr  & $^{88}$Sr &$^{88}$Sr  &$^{88}$Sr  & $^{88}$Sr &$^{62}$Ni   &$^{62}$Ni   &$^{62}$Ni  \\
 4&$^{88}$Sr  &$^{88}$Sr  &$^{88}$Sr  &$^{86}$Kr  &$^{86}$Kr   &$^{86}$Kr  &$^{86}$Kr  &$^{86}$Kr  & $^{86}$Kr &$^{86}$Sr  &$^{86}$Kr  &$^{86}$Kr  &$^{88}$Sr   &$^{88}$Sr   & $^{88}$Sr \\
 5&$^{86}$Kr  & $^{86}$Kr &$^{86}$Kr  &$^{84}$Se  & $^{84}$Se  &$^{84}$Se  &$^{84}$Se  &$^{84}$Se  & $^{84}$Se &$^{84}$Kr  &$^{84}$Se  &$^{84}$Se  &$^{86}$Kr   &$^{86}$Kr   &  $^{86}$Kr\\
 6&$^{84}$Se  &$^{84}$Se  &$^{84}$Se  &$^{82}$Ge  & $^{82}$Ge  &$^{82}$Ge  &$^{82}$Ge  &$^{82}$Ge  & $^{82}$Ge &$^{82}$Ge  &$^{82}$Ge  &$^{82}$Ge  &$^{84}$Se   & $^{84}$Se  &  $^{84}$Se\\
 7&$^{82}$Ge  &$^{82}$Ge &$^{82}$Ge  &$^{132}$Sn  &$^{132}$Sn  &$^{132}$Sn  &$^{132}$Sn  &$^{132}$Sn & $^{132}$Sn &$^{132}$Sn  &$^{132}$Sn  &$^{132}$Sn  &$^{82}$Ge   &$^{82}$Ge   &  $^{82}$Ge\\
 8&$^{80}$Zn  &$^{80}$Zn  &$^{80}$Zn  &$^{80}$Zn  &$^{80}$Zn   &$^{80}$Zn  &$^{130}$Cd   &$^{130}$Cd & $^{130}$Cd &$^{130}$Cd  &$^{130}$Cd  & $^{130}$Pd  &$^{132}$Sn   &$^{132}$Sn  &  $^{132}$Sn\\
 9&$^{78}$Ni  &$^{78}$Ni  &$^{78}$Ni  & $^{130}$Cd &$^{130}$Cd &$^{130}$Cd &$^{128}$Pd   & $^{128}$Pd & $^{128}$Pd &$^{128}$Pd &  $^{128}$Pd &$^{126}$Ru &$^{130}$Cd &$^{130}$Cd &$^{130}$Cd\\
 10&$^{126}$Ru  &$^{126}$Ru  &$^{126}$Ru  &$^{78}$Ni  &$^{78}$Ni     &$^{78}$Ni  &$^{126}$Ru &$^{126}$Ru  & $^{126}$Ru & $^{126}$Ru &$^{126}$Ru  &$^{124}$Mo  & $^{128}$Pd& $^{128}$Pd & $^{126}$Ru\\
 11&$^{124}$Mo  &$^{124}$Mo  &$^{124}$Mo  &$^{126}$Ru  &$^{126}$Ru   &$^{126}$Ru  &$^{124}$Mo  &$^{124}$Mo  & $^{124}$Mo &$^{124}$Mo  &$^{124}$Mo  &$^{122}$Zr  &$^{126}$Ru   &$^{126}$Ru   & $^{124}$Mo\\
 12&$^{122}$Zr  &$^{122}$Zr  &$^{122}$Zr  &$^{124}$Mo  &$^{124}$Mo   &$^{124}$mo  & $^{126}$Mo &$^{122}$Zr  & $^{122}$Zr &$^{126}$Mo  &$^{122}$Zr  &$^{120}$Sr  &$^{124}$Mo   &$^{124}$Mo   & $^{122}$Zr\\
 13&$^{124}$Zr  &$^{121}$Y  &$^{120}$Sr  &$^{122}$Zr  &$^{122}$Zr    &$^{122}$Zr  &$^{122}$Zr  &$^{124}$Zr  &$^{120}$Sr &$^{122}$zr   &$^{124}$Zr  &$^{118}$Kr  &$^{126}$Mo   &$^{122}$Zr   & $^{120}$Sr\\
 14&$^{120}$Sr  &$^{120}$Sr  &$^{118}$Kr  &$^{124}$SZr  &$^{124}$Zr  &$^{120}$Sr  &$^{124}$Zr  &$^{120}$Sr  &$^{118}$Kr &$^{124}$Zr  &$^{120}$Sr  &             &$^{122}$Zr   &$^{124}$Zr   & \\
 15&$^{122}$Sr  &$^{122}$Sr  &            &$^{120}$Sr  &$^{120}$Sr   &$^{118}$Kr  &$^{122}$Sr  &$^{122}$Sr  &           &$^{122}$Sr  &$^{122}$Sr  &             &$^{124}$Zr   &$^{120}$Sr   & \\
16&$^{124}$Sr  & $^{124}$Sr &             &$^{122}$Sr  &$^{122}$Sr   &            &$^{124}$Sr  & $^{124}$Sr &           & $^{124}$Sr &$^{124}$Sr  &             &$^{122}$Sr   &$^{122}$Sr   & \\
17&$^{126}$Sr  &            &             &$^{124}$Sr  &$^{124}$Sr   &            &$^{126}$Sr  &            &           &$^{126}$Sr  & $^{178}$Te &             &$^{124}$Sr   &$^{180}$Xe   & \\
18&            &            &             &$^{126}$Sr  &            &             &            &            &           &            &            &             &$^{178}$Te   &$^{178}$Te   & \\
\hline
\hline
\end{tabular}%
}     
\end{table*}

\end{comment}
%%%%%%%%%%%


==> titlepage_synopsis.tex <==
\begin{titlepage}
\thispagestyle{empty}
   \begin{center}
       \vspace*{1cm}
       \textbf{\large A STUDY OF EXOTIC COMPOUND NUCLEAR SYSTEMS AND SUBSEQUENT FRAGMENT EMISSION USING SKYRME ENERGY DENSITY FORMALISM}%Thesis Title

       \vspace{0.5cm}
       \textit{\large A THESIS}
        % Thesis Subtitle %Thesis Subtitle
       
       \vspace{0.10cm}
       Submitted for the partial fulfillment of requirement for the award of the degree of
       
       \vspace{0.20cm}
       \textit{\large DOCTOR OF PHILOSOPHY}
       
       \vspace{0.20CM}
       By
       
       \textbf{\LARGE Shivani Jain\\ \small( Reg. No: 901612016)}%Author Name
       
       \vspace{0.20cm}
       \textit{\large Under the supervision of}
       
\begin{minipage}[t]{7cm}
\flushleft
\textbf{Dr. Manoj K. Sharma}\\
Professor
\end{minipage}
\hfill
\begin{minipage}[t]{7cm}
\flushright
\textbf{Dr. Raj Kumar}\\
Associate Professor
\end{minipage} 
\newline
\centering{\includegraphics[scale=1.5]{images/TIET_logo.eps}}
\vspace*{0.8cm}        
\\SCHOOL OF PHYSICS AND MATERIALS SCIENCE\\
          THAPAR INSTITUTE OF ENGINEERING AND TECHNOLOGY, PATIALA - 147004\\
          PUNJAB, INDIA\\
          JUNE-2022
   \end{center}
\end{titlepage}

